Formation of black widows through ultra-compact X-ray binaries with He star companions

Black widows (BWs) are a type of eclipsing millisecond pulsars (MSPs) with companion masses $M_2$ $\lesssim 0.05\,\rm M_\odot$, which can be used to study the accretion history and the radiation of pulsars, as well as the origin of isolated MSPs. Recent observations indicate that there are two sub-types of BWs. One is the BWs with $M_2$ $\sim$ $0.01-0.05\,\rm M_\odot$, whereas another with $M_2$ $\lesssim 0.01\,\rm M_\odot$. However, the origin of the latter is still highly uncertain. In this paper, we investigated the formation of BWs with $M_2$ $\lesssim 0.01\,\rm M_\odot$ through ultra-compact X-ray binaries (UCXBs) with He star companions, in which a neutron star (NS) accretes material from a He star through Roche-lobe overflow. By considering different He star masses and evaporation efficiencies with the stellar evolution code Modules for Experiments in Stellar Astrophysics (MESA), we evolved a series of NS+He star systems that can undergo UCXB stage. We found that this channel can explain the formation of BWs with $M_2$ $\lesssim 0.01\,\rm M_\odot$ within the Hubble time, especially three widely studied BWs, i.e. PSRs J1719-1438, J2322-2650 and J1311-3430. We also found that X-ray irradiation feedback does not affect the evolutionary tracks of evaporation process. Our simulations indicate that the UCXB channel with He star companions are the potential progenitors of isolated MSPs, and that the origin of BWs with $M_2$ $\lesssim 0.01\,\rm M_\odot$ is different with another sub-type of BWs. In addition, the present work suggests that the BWs with $M_2$ $\lesssim 0.01\,\rm M_\odot$ may not be produced by redback systems.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

